How much do language models memorize?

We propose a new method for estimating how much a model knows about a datapoint and use it to measure the capacity of modern language models. Prior studies of language model memorization have struggled to disentangle memorization from generalization. We formally separate memorization into two components: unintended memorization, the information a model contains about a specific dataset, and generalization, the information a model contains about the true data-generation process. When we completely eliminate generalization, we can compute the total memorization, which provides an estimate of model capacity: our measurements estimate that GPT-style models have a capacity of approximately 3.6 bits per parameter. We train language models on datasets of increasing size and observe that models memorize until their capacity fills, at which point "grokking" begins, and unintended memorization decreases as models begin to generalize. We train hundreds of transformer language models ranging from $500K$ to $1.5B$ parameters and produce a series of scaling laws relating model capacity and data size to membership inference.

==> main_old.tex <==

\section{Related Work}

\paragraph{Language model memorization.}

\paragraph{Language modeling and compression.}

\paragraph{Scaling laws and model capacity.}

\section{Measuring Kolmogorov Memorization}
Large language models have demonstrated surprising performance. Increasing their size, computational power, and the amount of training data makes them progressively better. However, a significant concern with this paradigm is our limited understanding of how much these models "memorize" the training data. The datasets used could be stored somewhere within the model's weights without our realization. 

We are interested in a notion of memorization that helps us address the following question:


\begin{framed}
\begin{quote}
\it
Given a message \( m \) and a model \( \theta \), is \( m \) memorized in \( \theta \)? If so, to what extent?
\end{quote}
\end{framed}
Note that this question is independent of the training algorithm used for training the model \( \theta \), as well as the training data used for training it. This makes the algorithmic notions of ``influence" unsuitable for us.

\paragraph{Previous Notions of Memorization}
We are not the first to explore this question. Previous work has studied it in the context of reconstruction attacks. \citet{carlini2019secretsharerevaluatingtesting} defined a string \( m \) as memorized by a language model \( \theta \) if the second half of \( m \) can be generated greedily when prompting the model with the first half. 

Following this, \citet{nasr2023scalableextractiontrainingdata} introduced the notion of \textit{extractable memorization}, where a model \( \theta \) is said to memorize a message \( m \) if an adversarial prompt \( p \) can be found that generates \( m \).

\citet{mireshghallah2022memorizationnlpfinetuningmethods} and then \citet{schwarzschild2024rethinkingllmmemorizationlens} refined this notion by restricting the prompt \( p \) to be shorter than a certain number of tokens, preventing the prompt from containing the entire message \( m \). This refinement aims to provide a more accurate and meaningful notion of memorization. However, it still has limitations. For example, generating the sequence "cat cat cat ... cat" with the prompt "repeat cat 1000 times" does not necessarily indicate memorization.

\TODO{Mention the carlini paper that uses gzip ratio to find memorization}


\section{Definitions}
In this work, we formulate a notion of memorization that we dub Kolmogorov memorization.



% \section{Memorization capacity}
% \begin{definition}We say a parameter space $\Theta$ has a memorization capacity on dataset of $cap_{f,f_b}(\Theta)$, if for all $\theta\in \Theta$ we have 
% $$\max_{x,\theta}\mathcal{KM}_f (\theta,x) \leq cap_{f,f_b}(\Theta).$$
% \end{definition}
% \begin{proposition}
% Let 
% \end{proposition}
% \paragraph{Why do we need a base description method?}
% \paragraph{What is a good relative description method?}
% \paragraph{What is a good base description method?}

% \paragraph{How much does the choice of the relative and base description methods matter?}
% \paragraph{Why is this a good way to measure memorization?}
% \paragraph{What are the implications of low or high memorization? How much memorization can a model with bounded parameters have? }
% \paragraph{What's the relation to other definitions of memorization?}


\section{What is memorization? The bits-in bits-out view.}
Imagine we have an oracle $O_\theta(.): \cX \to \cY$. This oracle is parameterized by $\theta$ and we hope to understand the extent of memorization in this oracle and its underlying parameters. You can think of this oracle as a greedy decoding of a language model on an input prompt for example. A prominent way to measure memorization of certain point $y\in \cY$ is to find a message $x$ such that $O_\theta(x)=y$, and then call $y$ memorized if such $x$ exists.
However, this view is flawed. The range of oracle might be the entire space and that cannot mean every element in $\cY$ is memorized. To address this, we put a restriction on the inputs. This restrictions should make sure that the ``information content'' in the input $x$ is not more than that of $y$. So then we call a message $y\in \cY$ memorized, iff
$$\exists x\in \cX;~~~\mathbf{IC}_{\cX}(x) \leq \mathbf{IC}_{\cY}(y);~~~ O_\theta(x)=y.$$

This view of memorization requires a well-defined notion of information content. The CMU paper (add proper citation) considers the greedy decoding oracle, and defines the information content of a string to be its length in tokens. However we argue both of these choices are not ideal.

\paragraph{Choice of the Oracle} Note that the bits-in bits-out view is an meaningful notion of memorization of a point $y$ in parameters $\theta$, regardless of how the oracle works. To get a sense of worst-case memorization, we would better off choosing the oracle that is optimized for memorization. We list several candidates for such an Oracle:

\begin{enumerate}
    \item Greedy decoding oracle: This oracle, which is used by the CMU paper, will take an input $x$ and output the greedy decoding of language model when given $x$ as a prefix and generates $y$. Then the oracle outputs $y$.

    \item Extended greedy decoding oracle: This Oracle, which is used in google's paper, will take an input $x$ and output the greedy decoding of language model when given $x$ as a prefix and generates $y$. Then the oracle outputs $(x,y)$. Note that the subtle difference in defining this oracle implies that $x$ itself should be part of the message that is being memorized. 

    \item Compression based oracles: The oracle can be completely different from how people use language models to generate text. For example, we can use arbitrary decoding algorithms with inputs that are not natural language. Arithmetic decoding is one such alternative. In this oracle, instead of making the input $x$ to be prompt a 
 natural language prompt, we use the arithmetic code. Then the Orcale is defined by $O_\theta(x) = \mathbf{arithmetic-decode}(\theta, x).$
 So, to find an $x$ such that $O_\theta(x) =y$, we only need to encode $y$ using arithmetic coding, namely, $x=\mathbf{arithmetic-code}(\theta, y).$
\end{enumerate}
\paragraph{Measuring information content} A key challenge in realizing the notion of memorization through the bits-in bits-out view is how to measure the information content. A very simplistic way is to look at the bit length, Bit-length unfortunately cannot represent the true information content when the content is not represented in its most compressed form. An ideal notion of information content would measure the number of bits needed to represent the content in its ``most compressed form``. Moreover, we note that the right measure of information content is relative. For example, if we provide a look up table that maps indexes to images, and measure the information content of an image relative to this table, then, the most compressed form of storing an image relative to this table is to store the index. Similarly, for language data, we can define the information content relative to the structure of the language. This relativization helps us to separate memorization from generalization. To make this notion concrete, we use the notion of relative Kolmogrov complexity.

\begin{definition}
    [Relative description method]
    Let $\Sigma$ be an arbitrary alphabet and $\Theta$ an arbitrary space. We call a (partial) function $f\colon \Sigma^* \times \Theta \to \Sigma^*$ a relative description method. We say $p\in \Sigma^*$ is a the description of input $x$, relative to $\theta\in \Theta$, under the description method $f$, if we have
    $f(p,\theta)=x$.We also use $f(p)$ to refer to the case where no $\theta$ is provided and the description method works with a default $\theta$.
    We define several properties for a description method:

    \begin{itemize}
        \item{Completeness} We say a relative description method is complete iff
        $$\forall \theta\in \Theta, x\in \Sigma^*,  \exists p\in \Sigma^* \st f(p,\theta)=x.$$
        \item{Efficiency} TBD

    \end{itemize}
\end{definition}

\begin{definition} [Relative Kolmogorov complexity] 
Let $f\colon \Sigma^* \times \Theta \to \Sigma^* $ be a relative description method. We define the relative Kolmogorov complexity of an input $x$ with respect to $f$ and relative to a string $\theta\in \Theta$ is defined as 

$$\mathcal{KC}^\theta_{f}(x)=\min_{p\in \Sigma^*} \set{|p|;  f(p,\theta)=x}.$$
In case no $\theta$ is provided, the Kolmogrov complexity is defined as 

$$\mathcal{KC}_{f}(x)=\min_{p\in \Sigma^*} \set{|p|;  f(p)=x}.$$


\end{definition}
\begin{example}
Let $\Theta$ be the space of language models. Let $\theta\in \Theta$ be a specific language model. Define $f(p,\theta)$ to be the output of the language model $\theta$, when prompting it with a prompt $p$, using a specific decoding algorithm. Then $f$ is description method that we can define Kolmogorov complexity based off. Note that this description method is neither complete nor efficient. 
\end{example}

% We now define the notion of memorization 
% \begin{definition}[Kolmogorov memorization]
%     Let $\theta \in \Theta$ be a target model. Let $f\colon \Sigma^*\times \Theta \to \Sigma^*$ be an arbitrary description method. We define Kolmogorov memorization of a point $x$ in $\theta$, with respect to a description method $f$ to be defined as,
%     $$\mathcal{KM}_{f,f_b}(x,\theta) = {\mathcal{KC}_{f}(x)}-{\mathcal{KC}_{f}^{\theta}(x)}$$
% \end{definition}

\subsection{Memorization capacity}
After fixing the notion of memorization, we can now define a notion for can memorization capacity. 

\subsection{Implications of the bits-in bits-out perspective}

\paragraph{Prior work overestimates memorization.} Other prior work \citep{carlini2023quantifyingmemorizationneurallanguage} shows trends that for a fixed-length suffix, increasing prefix length will  increase the amount of extracted text. We show that this is not always true – increasing the prefix length also increases the number of bits in. \Cref{fig:memorization_comparison} compares Kolmogorov memorization to token-level memorization across the 10,000 most frequent documents in the Dolma corpus. We observe consistently lower memorization across model sizes and prompt lengths; interestingly, Kolmogorov memorization still increases with longer prompts.
\paragraph{GCG cannot find memorization.} We show that GCG can only find very high-entropy prefixes for relatively low-entropy outputs, meaning that it doesn't actually find memorization under our definition \citep{schwarzschild2024rethinkingllmmemorizationlens}; it's doing something more akin to passing secret messages to be decoded by the LM. \TODO{Jack - show this in a table, and give some more results about how GCG can't easily be adjusted to find memorization under this definition.}

\section{Experiments}
\subsection{Model capacity experiments}
We vary the model size, call the set of 
sizes $S=\set{s_1,\dots, s_k}$. For each model size $s_i$ we use a range of data sizes $D_i=\set{d^i_1,\dots, d^i_l}$. Then we train a a model $\theta_{i,j}$ with a model size $s_i$ dataset size $d^i_j$, making sure that the loss converges. We then measure the Kolmogrov memorization of the model $\theta_{i,j}$ on dataset $d_j$. Since $d_j$ is random, we do not need to carefully choose a base model as the information content of the dataset is known. We call this Kolmogorov memorization $k_{i,j}.$

\NOTE{10/23 We should measure both arithmetic coding size (loss) and prefix arithmetic coding size (new compression scheme?).}


\paragraph{What do we expect?} 
For a given model size $s_i$, the Kolmogrov memorization $k_{i,j}$ is increasing w.r.t $j$ but it will plateau to model's capacity. For any larger dataset than model's capacity. For larger model sizes, we expect this plateau happen on larger datasets and lead to greater model capacities.

\subsection{Training dynamics experiments}
\paragraph{Small models} We can use the same setup as our experiments above and ablate the effect of training dynamics on the memorization. 
\begin{enumerate}
\item{\textbf{Number of epochs}} See the effect of epochs of training on the Kolmogorov memorization of the entire dataset. 

\item{\textbf{Effect of number of repetitions on  memorization}} In this experiment, we devide the dataset into 10 bins, bin $i$ is repeated $i$ times. Then we train the model to convergence. We compare the kolmogorov memorization of different bins. The overall memorization should still add up to the model capacity, but distributed differently.

\item{\textbf{Effect of data order on memorization and forgetting}} Divide the data into two halfs. Train 100 epochs on the first half, then train 100 epochs on the second half, compare the kolmogrov memorization. \NOTE{Idea is that we have to forget some stuff since models have fixed capacity.}


\end{enumerate}
\paragraph{Large models and real data}
We can perform a limited number of experiments on fine-tuning large models with fine-tuning datasets. All the training dynamics discussed above would be interesting. 

\subsection{Detecting memorization in pre-training and fine-tuning data experiments}
These experiment compare our memorization metric with previous ones. 

\begin{enumerate}
    \item {\textbf{Population level experiments}}
    \item{\textbf{Worst-case experiments} Do we detect all of the LLM memorization benchmark data points as heavily memorized even if we cannot find the prompt?}
    \item{\textbf{Over-estimation of memorization memorization from previous work}}
\end{enumerate}


\section{Scaling laws for model capacity}

\Cref{lu2024scalinglawsfactmemorization} explored some semblance of scaling laws for model memorization...

What is the \textit{total} number of bits that can be stored in a language model? Given our proof that language models can store only a bounded number of bits, we consider how much storage capacity that contemporary Transformers might contain across model scales.

\clearpage
\bibliography{refs}
\bibliographystyle{alpha}
\bibliography{sample}
\appendix

\paragraph{Membership Inference as an Artifact of Memorization}

Researchers have used membership inference attacks to demonstrate memorization in language models and other machine learning models. Specifically, given a model \( \theta \) and a message \( m \) sampled from either the training set or the validation set with equal probability, the attack attempts to determine whether \( m \) is from the training or validation set. Successful membership inference is considered a sign of memorization.

However, a successful membership inference attack does not need to reconstruct the message \( m \); it only needs to output a bit, making the attack simpler. A problem with membership inference attacks on large models is that they often fail in the average case because most modern models do not memorize all of their training data. Researchers have suggested looking at the precision-recall curve for membership inference attacks to avoid a false sense of privacy (or lack of memorization), as this curve provides a worst-case sense of memorization.

Membership inference cannot answer our main question, as it requires access to the training set, while our question is independent of it. What does it mean if a membership inference attack infers that a message \( m \) is a member of the training set for model \( \theta \) with an average accuracy of 50.1? %? Should we conclude that this message is memorized? To what extent is it memorized?

A new notion of memorization for several reasons:
\begin{itemize}
\item{Privacy} When models are trained on private and sensitive data, what is the risk of the training data being leaked through the model's weights or its black-box behavior?
\item{Copyright} How can we gauge the extent to which a particular example has influenced a model? Measuring memorization for a specific training point could serve as evidence for or against copyright violation.
\item{Memory in language models} How much of a language model's performance is due to its memory capacity versus its computational capacity? Accurately measuring memory and memorization brings us closer to answering this question.
\end{itemize}

\paragraph{Our contributions}

- Our new definition without the problems and unifies all the previous notions of memorization in the context of compression.\\

-Enables defining memorization capacity of different architectures.\\
- Through our notion of memorization and model capacity, we identify why membership inference attacks cannot and do not succeed. 


\paragraph{Tasks}
\begin{itemize}
\item Talk about the second model compression and the effect what the effect of the base information on the definition.

\item Design experiments to show that our notions makes sense intuitively.\\
    - Detect false positives from previous work.\\
    - Fine tune models and see the dynamics of memorization \\
\end{itemize}

\TODO{As discussed on 10/22 and 10/5, it would be nice to have finetuning results. We could essentially show that finetuning follows fixed rules and we can only memorize a fixed number of bits during finetuning, which scales with the number of steps. [Can you memorize all your finetuning data? Could we show how much of different popular datasets could be memorized?]}

\TODO{Add table showing visual examples of where ACR can't find a prompt but there is one, and where ACR finds a prompt but it's very strange/obviously too many bits.}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig1_memorization_comparison.png}
    \caption{Comparison of Memorization Techniques. All numbers are computed with outputs of length $50$ across the 10,000 most common documents of The Pile. }
    \TODO{Could we fit the CMU paper into this table too?}
    \label{fig:memorization_comparison}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/fig0_capacity_scale.png}
    \caption{Capacity}
    \label{fig:memorization_comparison}
\end{figure}






\begin{figure}[t]
    \centering
    \begin{minipage}{0.58\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/fig3_memorization_vs_params.png}
        \caption{Memorization vs Parameters}
        \label{fig:memorization_vs_params}
    \end{minipage}\hfill
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/fig4_storage_capacity.png}
        \caption{Storage Capacity}
        \label{fig:storage_capacity}
    \end{minipage}
\end{figure}

\input{tables/table01-gcg-info.tex}

==> plot_utils_code.tex <==

from typing import Optional, Union

import matplotlib
import matplotlib.font_manager as fm
import matplotlib.pyplot as plt
import numpy as np
import pandas as pd
import seaborn as sns


font_name = "Helvetica Neue LT Pro"

# colors = [
#     (0.5, 0.0, 0.13),  # Maroon
#     (0.6, 0.1, 0.2),   # Dark red
#     (0.7, 0.2, 0.3),   # Deep rose
#     (0.7, 0.8, 0.9),   # Pastel blue
#     (0.6, 0.7, 0.85),  # Light pastel blue
#     (0.5, 0.6, 0.8),   # Medium pastel blue
#     (0.4, 0.5, 0.7)    # Soft indigo
# ]
# def _get_capacity_cmap() -> matplotlib.colors.LinearSegmentedColormap:
#     return matplotlib.colors.LinearSegmentedColormap.from_list("PinkBlue", colors)

# def _get_capacity_palette(n_colors: int) -> sns.color_palette:
#     pink_blue_cmap = _get_capacity_cmap()
#     if n_colors == 1:
#         return [pink_blue_cmap(0.5)]
#     else:
#         palette = [pink_blue_cmap(i / (n_colors - 1)) for i in range(n_colors)]
#         return sns.color_palette(palette)


grid_color = "#A8A29E"
def _init_plot():
    # Set font and style
    plt.rcParams['font.family'] = 'sans-serif'
    plt.rcParams['font.sans-serif'] = [font_name]
    plt.figure(figsize=(10, 8))
    # sns.set_theme(style="white", font_scale=1.9, font=font_name, context="notebook")
    sns.set_theme(style="whitegrid", 
        font_scale=1.8, font=font_name, 
        context="notebook", 
        rc={
            "axes.facecolor": (250/255, 243/255, 235/255, 1.0),
            "grid.color": grid_color, 
            "grid.linewidth": 1.5
        },
    )

def _format_label(label: Union[str, list, tuple]) -> str:
    label_str_0 = label[0].replace(" ", "\\ ")
    label_str_0 = r'$\bf{' + label_str_0 + '}$'
    label_str_1 = label[1]
    label_str_1 = f'\n({label_str_1})'
    return label_str_0 + label_str_1

def plot_df(
        df: pd.DataFrame,
        x: str,
        save_path: str,
        logx: bool = True,
        logy: bool = True,
        y: Optional[str] = None,
        yticks: Optional[list] = None,
        yticklabels: Optional[list] = None,
        ylabel: Optional[str] = None,
        xlabel: Optional[str] = None,
        xlim: Optional[tuple] = None,
        ylim: Optional[tuple] = None,
        title: Optional[str] = None,
        legend_title: str = "",
        legend_loc = "upper right",
        legend_hide: bool = False,
        kind: str = "line",
        custom_legend_labels: Optional[dict] = None,
        augment_ax: Optional[callable] = None,
        **plot_kwargs
    ):
    _init_plot()
    # Plot using Seaborn
    if kind == "line":
        plot_func = sns.lineplot
        if "lw" not in plot_kwargs:
            plot_kwargs["lw"] = 3.2
    elif kind == "scatter":
        plot_func = sns.scatterplot
    elif kind == "hist":
        plot_func = sns.histplot
    else:
        raise ValueError(f"Unknown plot kind: {kind}")
    
    plot_kwargs["rasterized"] = True
    # Replace markers
    if "marker" in plot_kwargs:
        plot_kwargs["marker"] = "h"

    ax = plot_func(data=df, x=x, y=y, **plot_kwargs)

    if logx: ax.set_xscale("log")
    if logy: ax.set_yscale("log")
    if yticks is not None: ax.set_yticks([0.001, 0.01, 0.1, 1])
    if yticklabels is not None: ax.set_yticklabels(["0.1%", "1%", "10%", "100%"])
    if ylabel is not None: 
        if isinstance(ylabel, tuple) or isinstance(ylabel, list):
            ax.set_ylabel(_format_label(ylabel), fontweight="light", labelpad=4)
        else:
            ax.set_ylabel(ylabel, fontweight="bold", labelpad=4)
    if xlabel is not None:
        if isinstance(xlabel, tuple) or isinstance(xlabel, list):
            ax.set_xlabel(_format_label(xlabel), fontweight="light", labelpad=4)
        else:
            ax.set_xlabel(xlabel, fontweight="bold", labelpad=4)
        
    if title is not None: 
        title_size = ax.xaxis.label.get_fontsize()
        ax.set_title(title, fontweight="bold", fontsize=title_size, pad=8)
    
    # Customize xlim and ylim
    if xlim is not None: ax.set_xlim(xlim)
    if ylim is not None: ax.set_ylim(ylim)

    # Run custom functionality
    if augment_ax is not None:
        augment_ax(ax)
    
    # Some more customization
    # Hide top and right spine
    ax.spines['top'].set_visible(False)
    ax.spines['right'].set_visible(False)
    # Customize ticks
    ax.xaxis.set_ticks_position('bottom')
    ax.yaxis.set_ticks_position('left')
    # ax.tick_params(axis='both', which='major', labelweight='light')
    # tick_font_color = (75/255, 58/255, 40/255)
    tick_font_color = "#444"
    for tick in ax.get_xticklabels():
        tick.set_fontweight(300)
        tick.set_fontsize(tick.get_fontsize() * 0.85)
        tick.set_color(tick_font_color)
    for tick in ax.get_yticklabels():
        tick.set_fontweight(300)
        tick.set_fontsize(tick.get_fontsize() * 0.85)
        tick.set_color(tick_font_color)

    # Customize legend
    legend = ax.get_legend()
    if legend is not None:
        handles = legend.legend_handles
        labels = [text.get_text() for text in legend.texts]
        if custom_legend_labels is not None:
            new_labels = [custom_legend_labels.get(label, str(label)) for label in labels]
            legend = ax.legend(handles, new_labels, handletextpad=0.5, labelspacing=0.2, loc=legend_loc, framealpha=1, facecolor="white")
        else:
            legend = ax.legend(handles, labels, handletextpad=0.5, labelspacing=0.2, loc=legend_loc, framealpha=1, facecolor="white")
        legend.set_title(legend_title)
        legend_font_size = ax.xaxis.label.get_fontsize() * 0.75
        legend.get_title().set_fontsize(legend_font_size)
        legend.get_title().set_weight('bold')
        for text in legend.get_texts():
            text.set_fontsize(legend_font_size)
        legend.get_frame().set_linewidth(2)
        legend.get_frame().set_edgecolor('gray')

        if legend_hide:
            legend.remove()

    # Customize plot borders
    border_width = 3.0
    border_color = 'black'
    ax.spines['top'].set_linewidth(border_width)
    ax.spines['top'].set_edgecolor(border_color)
    ax.spines['right'].set_linewidth(border_width)
    ax.spines['right'].set_edgecolor(border_color)
    ax.spines['left'].set_linewidth(border_width)
    ax.spines['left'].set_edgecolor(border_color)
    ax.spines['bottom'].set_linewidth(border_width)
    ax.spines['bottom'].set_edgecolor(border_color)

    plt.tight_layout()
    plt.savefig(
        save_path, 
        format='pdf', 
        bbox_inches='tight', 
        dpi=300,
    )
    print(f"Saved plot to {save_path}.")
    plt.show()
    return ax


==> tables/table01_compression_scores.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\begin{tabular}{r|c|cccc}
\toprule
Text type & AC & \multicolumn{3}{c}{RLC} \\
$k$ & - & $1$ & $10$ & $10,000$ & \\  \midrule
Random                     &    &     \\
Generated w/ greedy suffix &    &     \\
Highly memorized           &    &     \\ \bottomrule
\end{tabular}
\end{table}

==> tables/table03_text_memorization_examples.tex <==
\begin{tabular}{llrrrrr}
\toprule
\midrule
 & s & TF-IDF & Loss & Loss (ref.) & Kolmogorov & Extracted \\
159459 & 人気エリアであるフォンニャに位置するRock & Roll Hostelは、ビジネス出張と観光のどちらにも最適なロケーションです。 � & 78553.72 & 0.35 & 3.33 & 2.98 & 63 \\
72191 & このトピックには0件の返信が含まれ、1人の参加者がいます。1 年、 6 ヶ月前に Dave Gant さんが最後の更新 & 71279.19 & 0.47 & 1.56 & 1.09 & 15 \\
233292 & Label: Living Records
Destroy All MonstersメンバーBen Millerによる自主レーベルからのソロCD-R。こちらは付属の抽象画をサウンド化したと & 68064.46 & 1.15 & 3.88 & 2.73 & 44 \\
211977 & 《左傳》記「崔氏側莊公于北郭。丁亥，葬諸士孫之里，四翣，不� & 60820.46 & 0.75 & 3.64 & 2.89 & 6 \\
244971 & 歡迎客人自備紋身圖案或要求本紋身店代客起圖， 設計起圖須 & 60018.53 & 0.55 & 2.70 & 2.16 & 8 \\
133571 & By 小森 栄治,向山 洋一
Read Online or Download 中学の理科「総まとめ」を7日間で攻略する本 「� & 59625.40 & 1.26 & 3.53 & 2.27 & 1 \\
222697 & 統合分析是將一些議題相關但彼此獨立的臨床實驗之研究結果(大� & 59624.37 & 0.60 & 2.33 & 1.73 & 36 \\
183931 & 在SIA-Smaart Pro的Real-Time Module实时模块上，将功能扩展，实时显示相位和Fixed Point Per Octave（ & 59128.54 & 1.37 & 3.33 & 1.95 & 4 \\
206388 & Progress in Intelligent Transportation Systems and IoT/M2M Communications: Markets, Standardization, Technologies
|出版日||ページ情報||英文 173 Pages
|インテリジェント交通システムお & 58953.67 & 1.86 & 2.36 & 0.50 & 8 \\
51840 & English Title: Kingdom Hearts: Chain of Memories
Japanese Title: キングダム ハーツ チェイン オブ メモリーズ — “Kingdom Hearts: Chain of Memories”
Author: Tomoco Kanemaki
Illustrator: Shiro & 58605.92 & 1.61 & 2.59 & 0.99 & 0 \\
25193 & אשכול זה הועבר לארכיון. נא לשאול שאלה חדשה אם יש לך צורך & 58420.30 & 0.71 & 2.08 & 1.37 & 0 \\
259410 & 在《易經》里单数为阳, 双数为阴. 我曾怀疑马来西亚政府也会 & 58382.40 & 0.74 & 2.72 & 1.98 & 7 \\
73047 & 「XXl c.ー21世紀人」第3回企画展 三宅一生ディレクション
21_21 DESIGN SIGHT 第３回企画展の & 57797.99 & 1.17 & 3.72 & 2.55 & 10 \\
140400 & 无敌神马在线观看 重装机甲 睿峰影院 影院 LA幸福剧本
时间：2020-12 & 57399.24 & 0.48 & 3.16 & 2.67 & 0 \\
139558 & 季末小邪 回复 dgutkai: 楼主 您好 可以把项目源码发我吗？ 可以付� & 56539.93 & 0.73 & 3.19 & 2.46 & 18 \\
37397 & בכל סדנא אפשר לזהות את הילדים שהוריהם מאפשרים חופש יצי� & 56478.18 & 0.57 & 1.98 & 1.41 & 18 \\
102357 & Ακαδημαϊκές Δημοσιεύσεις Μελών ΔΕΠ σε άλλα Ιδρύματα >
� & 56376.74 & 1.11 & 1.87 & 0.75 & 10 \\
175096 & Larry想和李华，还有她那些中国朋友多在一起玩儿，了解更多的中国文 & 56152.72 & 0.95 & 2.11 & 1.16 & 1 \\
234299 & Mark 5:18 wrote:καὶ ἐμβαίνοντος αὐτοῦ εἰς τὸ πλοῖον παρεκάλει αὐ & 55391.28 & 1.50 & 1.69 & 0.19 & 3 \\
170325 & בתחילה הייתי סקפטית לגבי השקעת כסף בשיווק אינטרנטי. & 55014.00 & 0.72 & 2.12 & 1.41 & 4 \\
\bottomrule
\end{tabular}
